A Two-Stage, Model-Based Reinforcement Learning Approach for Active Flow Control of Bluff Body Wakes

This paper develops a data-driven, output-feedback approach to the infinite-horizon optimal control of high-dimensional nonlinear systems with unknown and unstable equilibria, using sparse partial observations. The approach builds on the transfer-plus-regulation decomposition of the infinite-horizon problem: a finite-horizon nonlinear transfer drives the system into a region where the dynamics are well-approximated by a linear model about the unknown operating point, and an infinite-horizon linear regulator identified within that region completes stabilization. We extend this framework to the partially observed setting by combining an ARMA-based information-state construction with a two-stage control architecture: an iterative linear quadratic regulator (iLQR) approach on the information state drives the system to the equilibrium neighborhood, discovered implicitly without prior knowledge of the target, and a locally identified time-invariant ARMA model provides the infinite-horizon regulator for asymptotic stabilization. The method requires no adjoint solver, reduced-order model, or full-state access. We validate the approach on high-fidelity Navier-Stokes simulations of the cylinder wake at $\mathrm{Re}=100$ using only eight surface pressure sensors, an order of magnitude fewer than recent model-based RL methods. The controller achieves complete suppression of vortex-shedding-induced lift oscillations and a $44\%$ reduction in total drag relative to the uncontrolled baseline.

==> Algorithm.tex <==
% ============================================================
\section{Information-State based Data-driven Flow Control Approach}
\label{sec4}
% ============================================================
% ============================================================
\subsection{Force Coefficient Estimation from Sparse Pressure Sensors}
\label{subsec:force_est}
% ============================================================
The lift and drag coefficients $C_L$ and $C_D$ depend on the full surface pressure and shear-stress distribution, neither of which is directly accessible from the $n_p = 8$ surface pressure sensors. We approximate the \emph{pressure contributions} to these coefficients via trapezoidal quadrature over the sensor locations. Let $\{\theta_i\}_{i=1}^{n_p}$ denote the equally-spaced azimuthal positions of the sensors, with $\Delta\theta = 2\pi/n_p$. Then
\begin{align}
    \widehat{C}_D(\mathbf{p}_k)
        &= -\frac{R\,\Delta\theta}{q_\infty D}
           \sum_{i=1}^{n_p} p_i^{(k)}\cos\theta_i,
    \label{eq:cdhat} \\
    \widehat{C}_L(\mathbf{p}_k)
        &= -\frac{R\,\Delta\theta}{q_\infty D}
           \sum_{i=1}^{n_p} p_i^{(k)}\sin\theta_i,
    \label{eq:clhat}
\end{align}
where $p_i^{(k)}$ is the pressure at sensor $i$ at time step $k$, $R = D/2$ is the cylinder radius, $D = 1$ is the cylinder diameter, and $q_\infty = \tfrac{1}{2}\rho U_\infty^2$ is the free-stream dynamic pressure. These approximations omit the viscous (skin-friction)
contribution to drag; at $\mathrm{Re} = 100$, the pressure drag dominates the total drag, so Eqs.~\eqref{eq:cdhat}--\eqref{eq:clhat} provide
a physically consistent, computationally inexpensive surrogate.
In what follows, we define the two-dimensional observation used for control as
\begin{equation}
    \mathbf{z}_k \triangleq \bigl[\widehat{C}_D(\mathbf{p}_k),\,\widehat{C}_L(\mathbf{p}_k)\bigr]^\top \in \mathbb{R}^{n_z},
    \qquad n_z = 2,
\end{equation}
where $\mathbf{p}_k \in \mathbb{R}^{n_p}$ denotes the raw pressure-sensor vector.

% ============================================================
\subsection{Information-State Formulation}
\label{subsec:info_state}
% ============================================================
Since the full flow state $\mathbf{x}_k$ is inaccessible, we follow the ARMA-based information-state construction of~\cite{TNNLS_PODiLQR} and define the
augmented state
\begin{equation}
    \mathcal{Z}_k
        = \bigl[\mathbf{z}_k^\top,\,\mathbf{z}_{k-1}^\top,\,\ldots,\,
                \mathbf{z}_{k-q+1}^\top,\,u_{k-1},\,\ldots,\,
                u_{k-q_u+1}\bigr]^\top
        \in \mathbb{R}^{n_\mathrm{aug}},
    \label{eq:info_state}
\end{equation}
where $q$ and $q_u$ are the observation and control history lengths, and
$n_\mathrm{aug} = n_z q + n_u(q_u - 1)$.
Under mild observability conditions, $\mathcal{Z}_k$ captures sufficient
information to render the partially observed system~\eqref{eq:state_space}--\eqref{eq:obs}
effectively fully observed~\cite{TNNLS_PODiLQR}.
The ARMA model for $\mathcal{Z}_k$ takes the companion form
\begin{equation}
    \mathcal{Z}_{k+1} = \mathbf{A}_k\,\mathcal{Z}_k + \mathbf{B}_k\,u_k,
    \label{eq:arma_dyn}
\end{equation}
The companion matrices $\mathbf{A}_k$ and $\mathbf{B}_k$ take the
structured form shown in Eq.~\eqref{eq:companion}.
\begin{table*}[!tp]
\begin{align}
\setcounter{MaxMatrixCols}{20}
\underbrace{
\begin{bmatrix}
\delta \mathbf{z}_{k} \\ \delta \mathbf{z}_{k-1} \\ \vdots \\ \delta \mathbf{z}_{k-q+1} \\
\hline
\delta u_{k-1} \\ \vdots \\ \delta u_{k-q_u+1}
\end{bmatrix}}_{\delta\mathcal{Z}_k}
=
\underbrace{\begin{bmatrix}
\alpha^k_1 & \cdots & \alpha^k_q & \vline & \beta^k_2 & \cdots & \beta^k_{q_u} \\
I & \cdots & 0 & \vline & 0 & \cdots & 0 \\
\vdots & \ddots & \vdots & \vline & \vdots & \ddots & \vdots \\
0 & \cdots & 0 & \vline & 0 & \cdots & 0 \\
\hline
0 & \cdots & 0 & \vline & 0 & \cdots & 0 \\
\vdots & & \vdots & \vline & I & \ddots & \vdots \\
0 & \cdots & 0 & \vline & 0 & \cdots & 0
\end{bmatrix}}_{\mathbf{A}_k}
\underbrace{\begin{bmatrix}
\delta \mathbf{z}_{k-1} \\ \vdots \\ \delta \mathbf{z}_{k-q} \\
\hline
\delta u_{k-2} \\ \vdots \\ \delta u_{k-q_u}
\end{bmatrix}}_{\delta\mathcal{Z}_{k-1}}
+
\underbrace{\begin{bmatrix}
\beta^k_1 \\ 0 \\ \vdots \\ 0 \\
\hline
1 \\ 0 \\ \vdots \\ 0
\end{bmatrix}}_{\mathbf{B}_k}
\delta u_{k-1}
\label{eq:companion}
\end{align}
\end{table*}
The top $n_z$ rows of $\mathbf{A}_k$ (coefficients $\alpha^k_1,\ldots,\alpha^k_q$,
$\beta^k_2,\ldots,\beta^k_{q_u}$) and the leading entry of $\mathbf{B}_k$
($\beta^k_1$) are identified from data; the remaining rows are fixed companion-shift blocks that propagate the observation and control histories forward in time.
\begin{remark}
    Although the discretized wake dynamics are extremely high-dimensional, cylinder wakes are well-known to evolve on low-dimensional manifolds dominated by a small number of coherent structures, as evidenced by POD- and balanced-POD-based reduced-order models (\cite{noack2003hierarchy,rowley2005model,willcox2002balanced}). This structure suggests that only a modest amount of input-output history may be needed to form an approximately Markov information state for prediction and control. Consistent with this intuition, we use short histories ($q=3$, $q_u=3$) throughout (Tables~\ref{tab:params_stage1}, \ref{tab:params_stage2}).
\end{remark}

% ============================================================
\subsection{Stage~I: POD-iLQR Global Transfer}
\label{subsec:stage1}
% ============================================================
The first stage applies the POD-iLQR algorithm to solve the finite-horizon optimal
control problem
\begin{equation}
    \min_{\{u_k\}_{k=0}^{N-1}}
    \sum_{k=0}^{N-1} c\bigl(\mathcal{Z}_k, u_k\bigr)
    + c_N\bigl(\mathcal{Z}_N\bigr),
    \label{eq:fhocp}
\end{equation}
with horizon $N = 50$ steps (25\,s at $\Delta t = 0.5$\,s).
POD-iLQR is an iterative procedure that alternates between a forward
simulation pass, an ARMA LTV system identification step, a backward
dynamic programming pass, and a control update. We summarize each step
below for completeness.
The running cost takes the form
$c(\mathcal{Z}_k, u_k) = \mathcal{Z}_k^\top Q\,\mathcal{Z}_k + u_k^\top R\,u_k$,
where $Q$ is block-diagonal over the observation history with an asymmetric
weighting that penalizes $\widehat{C}_L$ more heavily than $\widehat{C}_D$,
reflecting that $\widehat{C}_L = 0$ is a hard equilibrium condition while
$\widehat{C}_D$ is treated as a soft performance objective. A scaled terminal cost $c_N$
strongly incentivizes the trajectory to approach the unknown equilibrium
by the end of the horizon.

\subsubsection*{Step 1: Forward Pass}
Given the current nominal control sequence
$\bar{\mathbf{u}} = \{{\bar{u}_k}\}_{k=0}^{N-1}$, the PyFR simulator is
rolled out from the initial flow state to produce the nominal
information-state trajectory
$\bar{\mathcal{Z}} = \{\bar{\mathcal{Z}}_k\}_{k=0}^{N}$.

\subsubsection*{Step 2: ARMA LTV System Identification}
At each iLQR iteration, the LTV matrices
$\{\mathbf{A}_k,\mathbf{B}_k\}_{k=0}^{N-1}$ in~\eqref{eq:arma_dyn}
are identified from $n_\mathrm{samp}$ short rollouts launched from the
nominal trajectory. Random control perturbations $\delta u_k$ are
superimposed on $\bar{u}_k$; the resulting information-state deviations
$\delta\mathcal{Z}_k = \mathcal{Z}_k - \bar{\mathcal{Z}}_k$ are collected
across all rollouts and fitted by SVD-truncated least squares, independently
at each time step $k$, to obtain the companion matrices in~\eqref{eq:arma_dyn}.

\subsubsection*{Step 3: Backward Pass}
With the identified LTV model, a backward Riccati recursion is solved from $k = N$ to $k = 0$. Starting from the terminal value function $V_N(\delta\mathcal{Z}) = \delta\mathcal{Z}^\top Q_N \delta\mathcal{Z}$,
the value-function matrices $P_k$ and the gains are computed as
\begin{align}
    Q_{uu,k} &= R + \mathbf{B}_k^\top P_{k+1} \mathbf{B}_k, \\
    \mathbf{K}_k &= -Q_{uu,k}^{-1}\,\mathbf{B}_k^\top P_{k+1} \mathbf{A}_k, \\
    \mathbf{k}_k &= -Q_{uu,k}^{-1}\,\mathbf{B}_k^\top \mathbf{p}_{k+1},
\end{align}
where $\mathbf{p}_k$ is the value-function gradient and $P_k$ is updated via the standard discrete-time Riccati recursion.

\subsubsection*{Step 4: Control Update}
The nominal control sequence is updated as:
% \begin{equation}
    $u_k \leftarrow \bar{u}_k
        + \alpha\,\mathbf{k}_k
        + \mathbf{K}_k\,\bigl(\mathcal{Z}_k - \bar{\mathcal{Z}}_k\bigr)$,
    \label{eq:ilqr_update}
% \end{equation}
where $\alpha \in (0,1]$ is the line-search step size. Steps 1--4 are
repeated until convergence.

\subsubsection*{Transfer Outcome}
At the end of the iLQR horizon, the flow has been driven from sustained
periodic shedding to the neighborhood of the unknown equilibrium.
The terminal drag value
% \begin{equation}
    $\widehat{C}_D^* \triangleq \widehat{C}_D\!\left(\mathbf{p}_N\right)$
    \label{eq:cdstar}
% \end{equation}
is recorded as the drag level achieved at the end of the finite-horizon transfer.
Crucially, $\widehat{C}_D^*$ is discovered implicitly by the nonlinear optimizer and does not require prior knowledge of the
equilibrium state $\mathbf{x}^*$.

% ============================================================
\subsection{Stage~II: ARMA-LQR Local Stabilization}
\label{subsec:stage2}
% ============================================================
The second stage identifies an LTI model around the terminal operating
point and designs an LQR regulator to complete stabilization to the
unknown equilibrium. This stage implements the \emph{regulation}
component of the transfer-plus-regulation framework
in the data-driven, output-feedback setting.

\subsubsection*{LTI System Identification}
Starting from the terminal PyFR snapshot at time $t_N$, we execute
$n_r$ independent short rollouts of horizon $H$ steps under small random
control perturbations with standard deviation $\sigma$. The information-state
deviations from the terminal operating point are collected, and a single
time-invariant companion pair $(\mathbf{A}, \mathbf{B})$ is fitted by
SVD-truncated least squares across all transitions from all rollouts:
\begin{equation}
    \delta\mathcal{Z}_{k+1}
        = \mathbf{A}\,\delta\mathcal{Z}_k + \mathbf{B}\,\delta u_k,
    \label{eq:lti_model}
\end{equation}
where $\delta\mathcal{Z}_k = \mathcal{Z}_k - \mathcal{Z}^*$ denotes the
deviation from the (zero) regulation reference $\mathcal{Z}^* = \mathbf{0}$, i.e.,
$\mathbf{z}^* = [0,\,0]^\top$ in $(\widehat{C}_D,\widehat{C}_L)$ coordinates.
All lagged observation and control slots are initialized to their corresponding
values at the terminal snapshot. The SVD truncation retains singular values that
explain 99.99\% of the total energy, suppressing poorly excited directions
without introducing bias.

\subsubsection*{LQR Design}
Given the identified model $(\mathbf{A},\mathbf{B})$, the
infinite-horizon LQR gain is computed by solving the
Discrete Algebraic Riccati Equation (DARE):
\begin{equation}
    \mathbf{K} = \bigl(R_\ell + \mathbf{B}^\top P\mathbf{B}\bigr)^{-1}
                 \mathbf{B}^\top P\,\mathbf{A},
    \label{eq:lqr_gain}
\end{equation}
where $P$ satisfies the DARE for the pair $(\mathbf{A},\mathbf{B},Q_\ell,R_\ell)$.
The weight matrices $Q_\ell$ and $R_\ell$ follow the same block-diagonal
structure as Stage~I but with increased asymmetry toward $\widehat{C}_L$
and a relaxed control penalty, giving the regulator greater authority in
the local linear regime (see Table~\ref{tab:params_stage2}).
The resulting output feedback law is
\begin{equation}
    u_k = -\mathbf{K}\,\bigl(\mathcal{Z}_k - \mathcal{Z}^*\bigr),
    \label{eq:lqr_law}
\end{equation}
which drives the information-state, and hence the force coefficients
$(\widehat{C}_D, \widehat{C}_L)$, toward the setpoint $(0, 0)$ in the quadratic objective.

\begin{remark}
    The regulation reference $\mathcal{Z}^*$ is fixed at zero, while the local ARMA model used in Stage~II is identified from rollouts initialized at the terminal Stage~I snapshot, i.e., within the equilibrium neighborhood reached by the transfer stage. This enables local stabilization without requiring knowledge of the full equilibrium state $\mathbf{x}^*$.
\end{remark}

==> ILQR.tex <==
\subsection{Iterative Linear Quadratic Regulator Details}

% The Iterative LQR algorithm implemented here is a variation of the classical Differential Dynamic Programming(DDP) algorithm, wherein we constrain ourselves to just the first derivative of the dynamics.
% Let $U_t=\{u_i\}_{i=t}^{T-1}$. The cost-to-go is, thus, defined as
% \begin{equation*}
%     J_t(x,U_t)=\sum_{i=t}^{T-1} c(x_t, u_t)+\phi(x_T)
% \end{equation*}

% The value function at time \textit{t} is the cost-to-go given the minimising control sequence,
% \begin{equation*}
%     V_t(x) \equiv \min_{U_t} J_t(x, U_t).
% \end{equation*}

% Setting $V_T(x)=\phi(x_T)$, we can apply the Dynamic Programming Principle, which reduces the minimization over a sequence of controls to a sequence of minimizations over a single
% control, proceeding backwards in time:
% \begin{align*}
%     V_t(x)=\min_{u_t} [c(x_t,u_t)+V_{t+1}(f(x_t,u_t))], \\
%     Q_t(x)=arg\min_{u_t} [c(x_t,u_t)+V_{t+1}(f(x_t,u_t))]
% \end{align*}
% We define the action-value function as a function of perturbations around the pair $(x_t, u_t)$:
% \begin{align*}
%     Q_t(\delta x_t, \delta u_t)=c(x_t+\delta x_t, u_t+\delta u_t)-c(x_t, u_t) +\\
%     V_{t+1}(f(x_t+\delta x_t, u_t+\delta u_t))-V_{t+1}(f(x_t, u_t))
% \end{align*}
% and expand to the second order
% \begin{align}
%     Q_t(\delta x_t, \delta u_t) \approx \frac{1}{2}\begin{bmatrix}
%     1\\
%     \delta x_t\\
%     \delta u_t
%     \end{bmatrix}^T \begin{bmatrix}
%     0 &Q_x^T &Q_u^T\\
%     Q_x &Q_{xx} &Q_{xu}\\
%     Q_u &Q_{ux} &Q_{uu}
%     \end{bmatrix} \begin{bmatrix}
%     1\\
%     \delta x_t\\
%     \delta u_t
%     \end{bmatrix}
% \label{eq:ilqg_2nd_order}
% \end{align}
% The expansion coefficients can be written as 
% \begin{align}
%     &Q_x = c_x+f_{x}^T V'_{x} \label{eq:ilqg1} \\
%     &Q_u = c_u+f_{u}^T V'_{u} \label{eq:ilqg2} \\
%     &Q_{xx} = c_{xx}+f_{x}^T V'_{xx}f_{x} + V'_x \cdot f_{xx}  \label{eq:ilqg3} \\
%     &Q_{ux} = c_{ux}+f_{u}^T V'_{xx}f_{x}  + V'_x \cdot f_{ux} \label{eq:ilqg4} \\
%     &Q_{uu} = c_{uu}+f_{u}^T V'_{xx}f_{u}  + V'_x \cdot f_{uu}\label{eq:ilqg5} 
% \end{align}
% where $V' \equiv V_{t+1}$. The final terms in equations \ref{eq:ilqg3}, \ref{eq:ilqg4} and  \ref{eq:ilqg5} are ignored in ILQR. 

% Minimizing equation \ref{eq:ilqg_2nd_order} w.r.t. $\delta u$ gives
% \begin{equation}
%     \delta u^* = arg \min_{\delta u} Q_t(\delta x,\delta u) = -Q_{uu}^{-1}(Q_u+Q_{ux}\delta x)
% \end{equation}
% This gives an open-loop term $k=-Q_{uu}^{-1}Q_u$, along with the feedback gain term $K=-Q_{uu}^{-1}Q_{ux}$. Substituting the policy in equation \ref{eq:ilqg_2nd_order}, we have a quadratic model of the value function:
% \begin{align*}
%     &\Delta V(t) = -\frac{1}{2} Q_u Q_{uu}^{-1}Q_u \\ %\label{eq:ilqg1} \\
%     &V_x(t) = Q_x-Q_u Q_{uu}^{-1}Q_{ux} \\%\label{eq:ilqg2} \\
%     &V_{xx}(t) = Q_xx-Q_{xu} Q_{uu}^{-1}Q_{ux}  %\label{eq:ilqg3}
% \end{align*}

% The backward pass recursively computes the local quadratic models of $V(t)$ and ${k(t), K(t)}$. When the backward pass is completed, a forward pass of the algorithm then computes a new trajectory:
% \begin{align*}
%     &\hat{x}(0)=x(0) \\
%     &\hat{u}_t = u_t+k(t)+K(t)(\hat{x}(t)=x(t))\\
%     &\hat{x}(t+1)=f(\hat{x}(t), \hat{u}_t)
% \end{align*}


We present details of the D2C-ILQR algorithm in the following. The pseudo-code is given in Algorithm \ref{model_free_DDP_OL}. The `forward pass' and `backward pass' algorithms are summarized in Algorithms \ref{model_free_DDP_OL_FP} and \ref{model_free_DDP_OL_BP} respectively. Algorithm \ref{model_free_DDP_feedback} presents the DDP feedback algorithm used to calculate the optimal feedback gain. 
\begin{algorithm}[!ht]
\footnotesize
  \caption{\strut Open-loop trajectory optimization via model-free ILQR}
  {\bf Input:} Initial State - ${\bf x_0}$, System parameters - $\mathcal{P}$\;
  $m \gets 1$. ~~\CommentSty{/* Initialize the iteration number $m$ to 1.*/}\\
  $forward\_pass\_flag$ = true. \\
  \CommentSty{/* Run until the difference in costs between subsequent iterations is less an $\epsilon$ fraction of the former cost.*/}\\
  \While {$m==1$ {\textnormal{or}} $({\text cost}(\mathbb{T}_{nom}^{m})/{\text cost}(\mathbb{T}_{nom}^{m-1})) < 1 + \epsilon$}{
  \CommentSty{/*Each iteration has a backward pass followed by a forward pass.*/}\\
  \{$k^{m}_{0:N-1}, K^{m}_{0:N-1}$\}, $backward\_pass\_success\_flag$ $=$ Backward Pass($\mathbb{T}_{nom}^{m}$, $\mathcal{P}$).\\
  \If{backward\_pass\_success\_flag == true}{
      $\mathbb{T}_{nom}^{m+1}, forward\_pass\_flag$ $=$ Forward Pass($\mathbb{T}_{nom}^{m}$,$\{k^{m}_{0:N-1}, K^m_{0:N-1}\}$, $\mathcal{P}$).\\
      \While{forward\_pass\_flag == false}{
            $\mathbb{T}_{nom}^{m+1}, forward\_pass\_flag$ $=$ Forward Pass($\mathbb{T}_{nom}^{m}$,$\{k^{m}_{0:N-1}, K^m_{0:N-1}\}$, $\mathcal{P}$).\\
            Reduce $\alpha$ from $\mathcal{P}$.    
        }
      }
  \Else{
        Increase $\mu$ from $\mathcal{P}$.~~\CommentSty{/* Regularization step */}\\
    }
      $m \leftarrow m + 1$. \\
  $\mathbb{T}^{*}_{nom} \gets \mathbb{T}^{m+1}_{nom}$.\\
  }
  
  {\bf return $\mathbb{T}^{*}_{nom}$}\\
  \label{model_free_DDP_OL}
\end{algorithm}

\begin{algorithm}[!htp]
\footnotesize
 \caption{\strut Forward Pass}
  {\bf Input:} Nominal trajectory - $\mathbb{T}_{nom}^{k}$, previous iteration policy parameters - $\{k_{0:N-1}, K_{0:N-1}\}$ and system and cost parameters - $\mathcal{P}$.\
%   \CommentSty{/* Unpack the previous nominal trajectory.*/}\\
  $\{{\bar{x}_t^{prev}, \bar{u}_t^{prev}}\} \gets \mathbb{T}_{nom}^{k}$.\\
%   \CommentSty{/* Initialize time to 0.*/}\\
  $t \gets 0$.\\
  \While {$t < N$}{
    %\CommentSty{/*$\alpha$ is the line-search parameter.*/} \\
    \CommentSty{/*Simulate one step forward ($\alpha$ is the line-search parameter.)*/}
    \begin{equation*}
    \begin{split}
        {\bar{u}_{t}} &= {\bar{u}_t^{prev}} + \alpha k_t + K_{t} ({\bar{x}_t} - {\bar{x}_t^{prev}}),\\
        {\bar{x}_{t+1}} &= simulate\_forward\_step({\bar{x}_t}, {\bar{u}_t}).
        \end{split}
    \end{equation*}
    $t \leftarrow t + 1$. 
    }
  $\mathbb{T}_{nom}^{k+1}$ $\gets$ $\{{\bf \bar{x}_{0:N}}, {\bf \bar{u}_{0:N-1}}\}.$\\
  \If{$\mathbb{T}_{nom}^{k+1}$ to $\mathbb{T}_{nom}^{k}$ \textnormal{is acceptable}}{
    {\bf return} $\mathbb{T}_{nom}^{k+1}$, true.
  }
  \Else{
    {\bf return} $\mathbb{T}_{nom}^{k}$, false.
  }
  \label{model_free_DDP_OL_FP}
\end{algorithm}
%
\begin{algorithm}[!htp]
\footnotesize
  \caption{\strut Backward Pass}
  {\bf Input:} Nominal trajectory - $\mathbb{T}_{nom}^{k}$, previous iteration policy parameters - $\{k_{0:N-1}, K_{0:N-1}\}$, horizon - N and system and cost parameters - $\mathcal{P}$.\\
  \CommentSty{/* Backward pass starts from the final time-step i.e, N-1.*/}\\
  $t \gets N - 1$.\ \\
  Compute $J_{x_N}$ and $J_{x_N x_N}$ using boundary conditions.\\
  \CommentSty{/*Keep a copy of previous policy gains.*/}\\
  $k\_old \gets k_{0:N}$ {and}  $K\_old \gets K_{0:N}$.\\
  
  \While {$t >= 0$}{
  \CommentSty{/*Obtain the Jacobians from simulator rollouts as shown in Section \ref{sys_id_solve}:*/}\\
  $f_{x_t}, f_{u_t} \gets model\_free\_jacobian({ \bar{x}_t},{\bar{u}_t}).$\\
  \CommentSty{/*Obtain the partials of the Q function as follows:*/}
    \begin{equation*}
    \begin{split}
    Q_{x_t} &= c_{x_t}  + h_{x_t}^T J_{x_{t+1}}^{\prime},\\
    Q_{u_t} &= c_{u_t} + h_{u_t}^T J_{x_{t+1}}^{\prime},\\
    Q_{x_t x_t} &= c_{x_t x_t} + h_{x_t}^T J_{x_{t+1} x_{t+1}}^{\prime} h_{x_t}, \\
    Q_{u_t x_t} &= c_{u_t x_t} + h_{u_t}^T (J_{x_{t+1} x_{t+1}}^{\prime} + \mu I_{n_x \times n_x}) h_{x_t}, \\
    Q_{u_t u_t} &= c_{u_t u_t} + h_{u_t}^T (J_{x_{t+1} x_{t+1}}^{\prime} + \mu I_{n_x \times n_x}) h_{u_t}.\\
    \end{split}
\end{equation*}
  \If{$Q_{u_t u_t}$ {\textnormal{is positive-definite}}}{
    \begin{equation*}
    \begin{split}
        k_t &= -Q_{u_t u_t}^{-1} Q_{u_t},\\
        K_t &= -Q_{u_t u_t}^{-1} Q_{u_t x_t}.
        \end{split}
    \end{equation*}
    }
    
%   \Endif
  \Else{
    \CommentSty{/*If $Q_{u_t u_t}$ is not positive-definite, then, abort the backward pass.*/}\\
    {\bf return } $\{ k\_old, K\_old\}$, false.
  }
  \CommentSty{/*Obtain the partials of the value function $J_t$ as follows:*/}
  \begin{equation*}
      \begin{split}
          J_{x_t} &= Q_{x_t} + K_{t}^T Q_{u_t u_t} k_t + K_t^T Q_{u_t} + Q_{u_t x_t}^T k_t,\\
          J_{x_t x_t} &= Q_{x_t x_t} + K_t^T Q_{u_t u_t} K_t + K_t^T Q_{u_t x_t} + Q_{u_t x_t}^T K_t.
      \end{split}
  \end{equation*}
  $t \leftarrow t - 1$ 
  }
  $k\_new = k_{0:N-1},$\\
  $K\_new = K_{0:N-1}.$\\
  {\bf return} $\{k\_new, K\_new\}$, true.
  \label{model_free_DDP_OL_BP}
\end{algorithm}

\begin{algorithm} [!htp]
\footnotesize
  \caption{\strut DDP Feedback}
  {\bf Input:} Nominal trajectory - $\mathbb{T}_{nom}^{k}$, horizon - N and system and cost parameters - $\mathcal{P}$.\\
  \CommentSty{/* Start from the final time-step i.e, N-1.*/}\\
  $t \gets N - 1$.\ \\
  Compute $J_{x_N}$ and $J_{x_N x_N}$ using boundary conditions.\\

  \While {$t >= 0$}{
  \CommentSty{/*Obtain the Jacobians from simulator rollouts as shown in Section \ref{sys_id_solve}:*/}\\
  $h_{x_t}, h_{u_t} \gets model\_free\_jacobian({ \bar{x}_t},{\bar{u}_t}).$\\
  \CommentSty{/*Obtain the Hessians from simulator rollouts as shown above:*/}\\
  $h_{x_tx_t}, h_{u_tx_t}, h_{u_tu_t} \gets model\_free\_hessian({ \bar{x}_t},{\bar{u}_t}).$\\
  \CommentSty{/*Obtain the partials of the Q function as follows:*/}
    \begin{equation*}
    \begin{split}
    Q_{x_t} &= c_{x_t}  + h_{x_t}^T J_{x_{t+1}}^{\prime},\\
    Q_{u_t} &= c_{u_t} + h_{u_t}^T J_{x_{t+1}}^{\prime},\\
    Q_{x_t x_t} &= c_{x_t x_t} + h_{x_t}^T J_{x_{t+1} x_{t+1}}^{\prime} h_{x_t} + J_{x_{t+1}}^{\prime}h_{x_tx_t}, \\
    Q_{u_t x_t} &= c_{u_t x_t} + h_{u_t}^T (J_{x_{t+1} x_{t+1}}^{\prime} + \mu I_{n_x \times n_x}) h_{x_t} + J_{x_{t+1}}^{\prime}h_{u_tx_t}, \\
    Q_{u_t u_t} &= c_{u_t u_t} + h_{u_t}^T (J_{x_{t+1} x_{t+1}}^{\prime} + \mu I_{n_x \times n_x}) h_{u_t} + J_{x_{t+1}}^{\prime}h_{u_tu_t}.\\
    \end{split}
\end{equation*}
  \If{$Q_{u_t u_t}$ {\textnormal{is positive-definite}}}{
    \begin{equation*}
    \begin{split}
        k_t &= -Q_{u_t u_t}^{-1} Q_{u_t},\\
        K_t &= -Q_{u_t u_t}^{-1} Q_{u_t x_t}.
        \end{split}
    \end{equation*}
    }
    
%   \Endif
  \Else{
    \CommentSty{/*If $Q_{u_t u_t}$ is not positive-definite, then, abort the backward pass.*/}\\
    {\bf return } error.
  }
  \CommentSty{/*Obtain the partials of the value function $J_t$ as follows:*/}
  \begin{equation*}
      \begin{split}
          J_{x_t} &= Q_{x_t} + K_{t}^T Q_{u_t u_t} k_t + K_t^T Q_{u_t} + Q_{u_t x_t}^T k_t,\\
          J_{x_t x_t} &= Q_{x_t x_t} + K_t^T Q_{u_t u_t} K_t + K_t^T Q_{u_t x_t} + Q_{u_t x_t}^T K_t.
      \end{split}
  \end{equation*}
  $t \leftarrow t - 1$ 
  }
  $K = K_{0:N-1}.$\\
  {\bf return} $\{K\}$, true.
  \label{model_free_DDP_feedback}
\end{algorithm}

% \subsection*{Estimation of Jacobians: Linear Least Squares by Central Difference (LLS-CD)}
% \label{sys_id_solve_supplementary}

% \textit{Note: The following is a more detailed discussion of section 4.1.1 in the main paper.}
% % We make a preliminary analysis on the number of evaluations required in the above algorithm. If the horizon is `$h$' and the number of iterations required to converge are `$n$', the algorithm requires us to estimate each of the $f_{\bf x_t}$ and $f_{\bf u_t}$ `$nh$' times. 


% % \begin{equation*}
% % \begin{split}
% %     &f({\bf \bar{x}_t} + \delta {\bf x_t}, {\bf \bar{u}_t} + \delta {\bf u_t}) = f({\bf \bar{x}_t}, {\bf \bar{u}_t}) + \begin{bmatrix} f_{\bf x_t}  f_{\bf u_t} \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \\ \delta {\bf u_t} \end{bmatrix} + \\&\frac{1}{2} \begin{bmatrix} \delta {\bf x_t}^T  \delta {\bf u_t}^T \end{bmatrix} \begin{bmatrix} f_{\bf x_t x_t}  f_{\bf x_t u_t}\\ f_{\bf u_t x_t}  f_{\bf u_t u_t}\end{bmatrix} \begin{bmatrix} \delta {\bf x_t} \\ \delta {\bf u_t}\end{bmatrix} +
% %     O(\| \delta {\bf x_t}\|^3 + \| \delta {\bf u_t}\|^3)\\
% %     &f({\bf \bar{x}_t} - \delta {\bf x_t}, {\bf \bar{u}_t} - \delta {\bf u_t}) = f({\bf \bar{x}_t}, {\bf \bar{u}_t}) - \begin{bmatrix} f_{\bf x_t} f_{\bf u_t} \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \\ \delta {\bf u_t} \end{bmatrix} + \\&\frac{1}{2} \begin{bmatrix} \delta {\bf x_t}^T \delta {\bf u_t}^T \end{bmatrix} \begin{bmatrix} f_{\bf x_t x_t}  f_{\bf x_t u_t}\\ f_{\bf u_t x_t}  f_{\bf u_t u_t}\end{bmatrix} \begin{bmatrix} \delta {\bf x_t} \\ \delta {\bf u_t}\end{bmatrix}+
% %     O(\| \delta {\bf x_t}\|^3 + \| \delta {\bf u_t}\|^3)\\
% %   \end{split}
% % \end{equation*}
% Using Taylor's expansions of `$h$' (for generality, $h$ is the non-linear model of Section 2) about the nominal trajectory $(\bar{x}_t,  \bar{u}_t)$ on both the positive and the negative sides, we obtain the following central difference equation:\\
% $
%     h(\bar{x}_t + \delta x_t, \bar{u}_t + \delta u_t) - h(\bar{x}_t - \delta x_t, \bar{u}_t - \delta  u_t) =~2 \begin{bmatrix} h_{x_t} & h_{u_t} \end{bmatrix} \begin{bmatrix}  \delta {x_t} \\ \delta {u_t} \end{bmatrix} + O(\| \delta {x_t}\|^2 + \| \delta {u_t}\|^2).
% $
% Multiplying by $\begin{bmatrix} \delta {x_t}^T & \delta {u_t}^T \end{bmatrix}$ on both sides to the above equation:
% \begin{equation*}
%     \begin{split}
%     \begin{bmatrix}h({\bar{x}_t} + \delta {x_t}, {\bar{u}_t} + \delta {u_t}) -  h({\bar{x}_t} - \delta {x_t}, {\bar{u}_t} - \delta {u_t})\end{bmatrix} 
%      \times \begin{bmatrix} \delta {x_t}^T & \delta {u_t}^T \end{bmatrix} 
%     % &= 2 \begin{bmatrix} f_{\bf x_t} & f_{\bf u_t} \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \\ \delta {\bf u_t} \end{bmatrix} \begin{bmatrix} \delta {\bf x_t}^T & \delta {\bf u_t}^T \end{bmatrix}+ O(\| \delta {\bf x_t}\|^4 + \| \delta {\bf u_t}\|^4)\\
%      =2 \begin{bmatrix} h_{x_t} & h_{u_t} \end{bmatrix} \begin{bmatrix}  \delta {x_t} \delta {x_t}^T & \delta {x_t} \delta {u_t}^T \\ \delta {u_t} \delta {x_t}^T  & \delta {u_t} \delta {u_t}^T \end{bmatrix} \nonumber \\~~~~~~~~~~~~
%      + O(\| \delta {x_t}\|^3 + \| \delta {u_t}\|^3)
%      \end{split}
% \end{equation*}
% Assuming that $\begin{bmatrix}  \delta {x_t} \delta {x_t}^T & \delta {x_t} \delta {u_t}^T \\ \delta {u_t} \delta {x_t}^T  & \delta {u_t} \delta {u_t}^T \end{bmatrix}$ is invertible (which will later be proved to be true by some assumptions), let us perform inversions on either sides of the above equation as follows:
% % \begin{equation*}
% %     \begin{split}
% %     &\begin{bmatrix}f({\bf \bar{x}_t} + \delta {\bf x_t}, {\bf \bar{u}_t} + \delta {\bf u_t}) - f({\bf \bar{x}_t} - \delta {\bf x_t}, {\bf \bar{u}_t} - \delta {\bf u_t})\end{bmatrix} \times\\
% %     &\begin{bmatrix} \delta {\bf x_t}^T & \delta {\bf u_t}^T \end{bmatrix} \begin{bmatrix}  \delta {\bf x_t} \delta {\bf x_t}^T & \delta {\bf x_t} \delta {\bf u_t}^T \\ \delta {\bf u_t} \delta {\bf x_t}^T  & \delta {\bf u_t} \delta {\bf u_t}^T \end{bmatrix}^{-1} = \\&2 \begin{bmatrix} f_{\bf x_t} & f_{\bf u_t} \end{bmatrix} +
% %      O(\| \delta {\bf x_t}\|^2 + \| \delta {\bf u_t}\|^2)
% %      \end{split}
% % \end{equation*}
% % $\implies$ 
% \begin{equation}
%     \begin{split}
%     \begin{bmatrix} h_{x_t}~h_{u_t} \end{bmatrix} 
%     &=\frac{1}{2}\begin{bmatrix} h({\bar{x}_t} + \delta {x_t}, {\bar{u}_t} + \delta {u_t}) - h({\bar{x}_t} - \delta {x_t}, {\bar{u}_t} - \delta {u_t})\end{bmatrix}  \times\begin{bmatrix} \delta {x_t}^T & \delta {u_t}^T \end{bmatrix} \begin{bmatrix}  \delta {x_t} \delta {x_t}^T~ \delta {x_t} \delta {u_t}^T \\ \delta {u_t} \delta {x_t}^T ~\delta {u_t} \delta {u_t}^T \end{bmatrix}^{-1}\\ &~~~~~~~~~~~~~~~~~~+ O(\| \delta {x_t}\| + \| \delta {u_t}\|)
%      \label{eq : model_free_DDP_jacobian_raw1}
%      \end{split}
% \end{equation}
% Equation \eqref{eq : model_free_DDP_jacobian_raw1} solves for Jacobians, $h_{x_t}$ and $h_{u_t}$, simultaneously. It is noted that the above formulation requires only 2 evaluations of $h(.)$, given the nominal state and control $\-$ (${\bar{x}_t},{\bar{u}_t}$). The remaining terms (also, the error in the evaluation) are of the order that is linear in $\delta {x_t}$ and $\delta {u_t}$. The following extends equation \eqref{eq : model_free_DDP_jacobian_raw1} to be used in practical implementations (sampling).\\
% We are free to choose the distribution of $\delta {x_t}$ and $\delta {u_t}$. We assume both are i.i.d. Gaussian distributed random variables with zero mean and a standard deviation of $\sigma$.~This ensures that $\begin{bmatrix}  \delta {x_t} \delta {x_t}^T & \delta {x_t} \delta {u_t}^T \\ \delta {u_t} \delta {x_t}^T  & \delta {u_t} \delta {u_t}^T \end{bmatrix}$ is invertible. Let `$n_s$' be the number of samples for each of the random variables, $\delta {x_t}$ and $\delta {u_t}$. Denote the random samples as $\delta {X_t} = \begin{bmatrix} \delta {x_t^1}& \delta {x_t^2}& \ldots &\delta {x_t^{n_s}}\end{bmatrix}$, $\delta {U_t} = \begin{bmatrix} \delta {u_t^1} &\delta {u_t^2}& \ldots& \delta {u_t^{n_s}}\end{bmatrix}$ and $\delta Y_t = \begin{bmatrix} \delta X_t & \delta U_t \end{bmatrix}$. Then $\begin{bmatrix} h_{x_t} & h_{u_t} \end{bmatrix}$ is given by the following (via standard least squares):
% \begin{equation}
%     \begin{split}
%     &\begin{bmatrix} h_{x_t}~h_{u_t} \end{bmatrix} = H \delta Y_t^T (\delta Y_t\delta Y_t^T)^{-1} \\
%     &H = \begin{bmatrix} h({\bar{x}_t} + \delta {x_t^1}, {\bar{u}_t} + \delta {u_t^1}) - h({ \bar{x}_t} - \delta {x_t^1}, {\bar{u}_t} - \delta {u_t^1})\\ h({\bar{x}_t} + \delta {x_t^2}, {\bar{u}_t} + \delta {u_t^2}) - h({\bar{x}_t} - \delta {x_t^2}, {\bar{u}_t} - \delta {u_t^2}) \\ \vdots  \\h({\bar{x}_t} + \delta {x_t^{n_s}}, {\bar{u}_t} + \delta {u_t^{n_s}}) - h({\bar{x}_t} - \delta {x_t^{n_s}}, {\bar{u}_t} - \delta {u_t^{n_s}})\end{bmatrix}
%      \label{eq : model_free_DDP_jacobian1}
%      \end{split}
% \end{equation}
% Let us consider the terms in the matrix $\delta Y_t \delta Y_t^T=\begin{bmatrix}  \delta {X_t} \delta {X_t}^T & \delta {X_t} \delta {U_t}^T \\ \delta {U_t} \delta {X_t}^T  & \delta {U_t} \delta {U_t}^T \end{bmatrix}$.~$\delta {X_t} \delta {X_t}^T = \sum_{i=1}^{n_s} \delta {x_t}^i {\delta {x_t}^i}^T$. Similarly, $\delta {U_t} \delta {U_t}^T = \sum_{i=1}^{n_s} \delta {u_t}^i {\delta {u_t}^i}^T$, $\delta {U_t} \delta {X_t}^T = \sum_{i=1}^{n_s} \delta {u_t}^i {\delta {x_t}^i}^T$ and $\delta {X_t} \delta {U_t}^T = \sum_{i=1}^{n_s} \delta {x_t}^i {\delta {u_t}^i}^T$. From the definition of sample variance, for a large enough $n_s$, we can write the above matrix as 
% \begin{equation*}
% \begin{split}
%     \delta Y_t \delta Y_t^T &= \begin{bmatrix} \sum_{i=1}^{n_s} \delta {x_t}^i {\delta {x_t}^i}^T & \sum_{i=1}^{n_s} \delta {x_t}^i {\delta {u_t}^i}^T \\ \sum_{i=1}^{n_s} \delta {u_t}^i {\delta {x_t}^i}^T & \sum_{i=1}^{n_s} \delta {u_t}^i {\delta {u_t}^i}^T
%     \end{bmatrix}\\ &\approx \begin{bmatrix} \sigma^2(n_s - 1) {\text I_{n_x}} & {\text 0_{n_x \times n_u}} \\ 0_{n_u \times n_x} & \sigma^2 (n_s - 1) {\text I_{n_u}}\end{bmatrix} \\
%     &= \sigma^2 (n_s - 1){\text I}_{(n_x+n_u) \times (n_x+n_u)}
% \end{split}
% \end{equation*}

% \textit{Sample Complexity.} 
% Given that we have high enough number of samples $n_s$, typically `$O(n_x + n_u)$', the above approximation holds good. The reason is as follows. Note that the above least squares procedure converges when the matrix $\delta Y_t \delta Y_t^T$ converges to the identity matrix. This is entirely equivalent to estimation of the covariance of the  random vector $[\delta x_t \ \delta u_t]$ where $\delta x_t$, and $\delta u_t$ are Gaussian i.i.d. samples. Thus, it follows that the number of samples is $O(n_x+n_u)$, given $n_x+n_u$ is large enough \cite{HDP-book}. \\
% Note that if one were to use an FD procedure, the number of samples would be $O(n_x(n_x+n_u)) >> O(n_x+n_u)$. In fact, this behaviour is clearly apparent in our empirical results where FD is more efficient for low dimensional examples, while the LLS-CD procedure rapidly becomes much more efficient as the size of the examples increases. This has very important ramifications since the overwhelming bulk of the computations in our D2C implementation is in the estimation of these system dynamics. 

% \subsection*{Guarantees for ILQR}
% %\textcolor{red}{Can you add the iLQR/ DDP insight here?}\\
% As has been mentioned previously, iLQR is much more efficient than the related DDP procedure \cite{ddp} which requires the availability of the second order dynamics terms. Albeit this is known empirically \cite{ilqg2}, it is not clear as to why iLQR should provide a solution of the same quality as DDP? \\
% The reasoning for this as follows. 
% The DDP procedure is simply a sequential quadratic programming (SQP) procedure for the trajectory optimization problem, where the dynamics are the constraints in the optimization problem. In SQP, the Lagrangian, i.e., the cost function augmented with the constraints using the Lagrange multipliers, $\mathcal{L}(x,\lambda) = c(x) + \lambda h(x)$, where $c(x)$ is the cost function and $h(x) =0$ are the constraints, is expanded to second order about the current solution. In the context of trajectory optimization, this amounts to expanding the cost function to second order which also results in second order expansion of the dynamics. The only difference between DDP and iLQR is that, in iLQR, the second order expansion of the dynamics is neglected in the optimization problem.
% This is similar to idea of neglecting second order terms in Gauss-Newton's method (identical to iLQR) as compared to Newton's method (identical to DDP).
% Moreover, the guarantees for SQP, i.e., convergence to a stationary point of the augmented cost function still holds for iLQR. Therefore, it follows that we can expect iLQR to converge to a stationary point of the optimal control problem.\\
% Next, note that due to the Method of Characteristics development in the previous section, if the dynamics are affine in control and the cost is quadratic in control, it follows that satisfying the necessary conditions for optimality, which iLQR is guaranteed to do under mild conditions, one is assured of the global minimum to the problem. Then, a perturbation expansion of the characteristic equations about this optimal is guaranteed to give us at least a local solution to the HJB equation.% due to Proposition~\ref{T-PFC}.
% %Since the inversion of an identity matrix is trivial and always exists, the above matrix is invertible in equation \eqref{eq : model_free_DDP_jacobian1}. Thus, one can calculate $f_{\bf x}$ and $f_{\bf u}$ this way during the backward pass. For the sake of convenience in the later sections, let us refer to this method as `Linear Least Squares by Central Difference (LLS-CD)'. 
% %The entire algorithm to determine the optimal nominal trajectory in a model-free fashion is summarized together in Algorithm \ref{model_free_DDP_OL}. The detailed forward and backward pass functions are shown in Algorithm \ref{model_free_DDP_OL_FP} and \ref{model_free_DDP_OL_BP} respectively in the supplementary material.

\subsection*{DDP Feedback Gain Calculation}
Once the optimal nominal trajectory is obtained with ILQR, one DDP back pass is conducted to find the linear optimal feedback gain as shown in Algorithm \ref{model_free_DDP_feedback}. Then the linear feedback is wrapped around the nominal control sequence ($u_t = \bar{u}_t + K_t\delta x_t$),where $\delta x_t$ is the state deviation from the nominal state $\bar{x}_t$.

% \sr
% \begin{align}
% z_i &= \begin{bmatrix} \delta {x}^T & \delta {u}^T \end{bmatrix} \begin{bmatrix} h_{xx}^{(i)}  & h_{xu}^{(i)}  \\ h_{ux}^{(i)}  & h_{uu}^{(i)}  \end{bmatrix} \begin{bmatrix}  \delta {x} \\ \delta {u} \end{bmatrix} \nonumber \\  \nonumber
% &= \sum_{j=1}^{n_s} \sum_{k=1}^{n_s} \dfrac{\partial^2 h_i}{\partial x_j \partial x_k} \delta x_j \delta x_k + 2 \sum_{p=1}^{n_u} \sum_{q=1}^{n_s} \dfrac{\partial^2 h_i}{\partial u_p \partial x_q} \delta u_p \delta x_q + \sum_{d=1}^{n_u} \sum_{h=1}^{n_u} \dfrac{\partial^2 h_i}{\partial u_d \partial u_h} \delta u_d \delta u_h \\ \nonumber
% &= \underbrace{\begin{bmatrix} \delta {x_1}^2 & \delta {x_1} \delta {x_2} & \cdots & \delta {x_1} \delta {u_{n_u}} & \delta {x_2}^2 & \delta {x_2} \delta {x_3} & \cdots& \delta {u^2_{n_u}}\end{bmatrix}}_{\delta {XU}}  \underbrace{\begin{bmatrix} \dfrac{\partial^2 h_i}{\partial x_1^2} \\ \\ 2 \dfrac{\partial^2 h_i}{\partial x_1 \partial x_2} \\ \vdots \\ 2 \dfrac{\partial^2 h_i}{\partial x_1 \partial u_{n_u}} \\ \\ \dfrac{\partial^2 h_i}{\partial x_2^2} \\ \\ 2 \dfrac{\partial^2 h_i}{\partial x_2 \partial x_3} \\ \vdots \\ \dfrac{\partial^2 h_i}{\partial {u^2_{n_u}}}\end{bmatrix}}_{H_i},\\
% \end{align}
% % \begin{bmatrix} \delta {x_1} & \delta {x_2} & \cdots & \delta {x_{n_s}} & \delta {u_1} & \delta {u_2} & \cdots & \delta {u_{n_u}} \end{bmatrix} 

% where $h_{xx}^{(i)} = \left.\dfrac{\partial^2 h_i}{\partial x^2}\right|_{x=t}$, $z_i$ is the $i^{th}$ element of vector $z_t$ and $h_i$ is the $i^{th}$ element of the dynamics vector $h(x_t, u_t)$. Multiplying on both sides by $\delta XU^T$ and apply standard Least Square method:
% $H_i = (\delta XU^T \delta XU)^{-1} \delta XU^T Z_i$. Then repeat for $i=1,2,...,n_s$ to get the estimation for the Hessian tensor.

==> Introduction_revised.tex <==
\section{Introduction}
Active flow control seeks to suppress wake unsteadiness (vortex shedding), oscillatory loads, and excess drag using feedback. The two-dimensional circular-cylinder wake is a canonical benchmark: above $\mathrm{Re}\approx 47$, the steady symmetric wake undergoes a Hopf bifurcation and transitions to periodic B\'enard--von K\'arm\'an shedding, increasing drag and inducing lift oscillations~\cite{williamson1996vortex,noack2003hierarchy}. Suppression therefore amounts to stabilizing the steady symmetric wake—an \emph{unstable equilibrium} that is not observed in open loop and whose location in the $O(10^5)$-dimensional state space is generally unavailable without specialized solvers. In addition, practical sensing is sparse (often only a few surface-pressure measurements). We thus address: \emph{stabilize an unknown unstable equilibrium using only partial observations, without an explicit model}, for which standard “regulate to a known setpoint” formulations are not applicable.

\begin{figure}[t]
\centering
\subfloat[Uncontrolled wake at $\mathrm{Re}=100$ (limit cycle).]{
  \includegraphics[width=0.7\linewidth]{figures/ilqr_norm1.png}
  \label{fig:intro_uncontrolled}
}\\
\subfloat[Controlled wake (equilibrium recovered).]{
  \includegraphics[width=0.7\linewidth]{figures/lqr_norm3.png}
  \label{fig:intro_controlled}
}
\caption{For $\mathrm{Re}>47$, open-loop dynamics converge to a vortex-shedding limit cycle; the desired steady wake is unstable.}
\label{fig:intro_motivation}
\vspace{-0.6cm}
\end{figure}

Classical wake-control methods typically build reduced-order models (e.g., POD/balanced truncation) and design controllers on them~\cite{rowley2005model,willcox2002balanced,bewley2001flow,Illingworth2016,Graham1999}, but require adjoints and/or full-state snapshots and are limited by basis fidelity. Deep reinforcement learning has also achieved suppression directly from interaction data~\cite{rabault2019artificial,tang2020robust,park2020deep,wang2024robust}, but model-free RL is sample-inefficient for high-fidelity CFD. Model-based RL improves sample efficiency by learning surrogates~\cite{ye2025mbrl,mao2024model,dong2023surrogate} but often uses high-capacity models, dense sensing (e.g., up to 151 probes~\cite{ye2025mbrl}), and yields feedback laws with limited analytical structure.

We propose a data-driven, output-feedback approach based on a \emph{transfer-plus-regulation} decomposition~\cite{mohamed2023optimal,mohamed2025optimal}. Stage~I performs finite-horizon nonlinear transfer to drive the flow from the shedding regime into the equilibrium neighborhood using iLQR on an ARMA-based information state. Stage~II identifies a local time-invariant ARMA model and designs an infinite-horizon LQR regulator for asymptotic stabilization. The method requires no adjoint solver, reduced-order model, or full-state access.

We validate on a high-order PyFR simulation~\cite{witherden2014pyfr} of the cylinder wake at $\mathrm{Re}=100$ ($n_x\approx 10^5$) using only eight surface pressure sensors. The controller fully suppresses lift oscillations and achieves a $44\%$ reduction in total drag (pressure+viscous, full surface integration) relative to the uncontrolled baseline.

The rest of the paper is organized as follows. Section~\ref{sec2} presents the governing equations and nonlinear optimal control formulation. Section~\ref{sec3} discusses the unknown-equilibrium and partial-observation challenges and introduces the output construction. Section~\ref{sec4} presents the information-state modeling and the two-stage POD-iLQR/ARMA-LQR design. Section~\ref{sec5} presents numerical experiments.
